Magnetically enhanced thin film coarsening by a magnetic XPFC model allowing to decouple magnetic anisotropy and magnetostriction

External magnetic fields provide a macroscopic control mechanism to influence the microstructure of polycrystalline materials. We model the influence of strong magnetic fields on grain growth in thin films with a magnetic extended phase field crystal (XPFC) model. The magneto-structural effects are incorporated into the correlation function in reciprocal space. With this approach magnetic anisotropy, magnetostriction and mobility of grain boundary can be controlled and a variety of geometrical and topological properties consistent with experimental results can be determined.

==> MyBibaliasAcite.tex <==
\makeatletter
% \bibalias{x}{y} makes \cite{x}
% equiv. to \cite{y}
\newcommand\bibalias[2]{%
\@namedef{bibali@#1}{#2}%
}

\newtoks\biba@toks
\newcommand\acite[2][]{%
\biba@toks{\cite#1}%
\def\biba@comma{}%
\def\biba@all{}%
\@for\biba@one:=#2\do{%
\@ifundefined{bibali@\biba@one}{%
\edef\biba@all{\biba@all\biba@comma\biba@one}%
}{%
\PackageInfo{bibalias}{%
Replacing citation `\biba@one' with `\@nameuse{bibali@\biba@one}'
}%
\edef\biba@all{\biba@all\biba@comma\@nameuse{bibali@\biba@one}}%
}%
\def\biba@comma{,}%
}%
\edef\biba@tmp{\the\biba@toks{\biba@all}}%
\biba@tmp
}

\makeatother

\bibalias{Athreya_PRE_2006}{AGD06}
\bibalias{Athreya}{AGD06}
\bibalias{Mullins_AM_1998}{Mul98}
\bibalias{Barmaketal_PMS_2013}{BEC13}
\bibalias{Backofenetal_PML_2007}{BRV07}
\bibalias{ReZaeietal_CMS_2021}{RJJ21}
\bibalias{Rezaeietal_CMS_2021}{RJJ21}
%
%
%
